A novel metric for detecting quadrotor loss-of-control

Unmanned aerial vehicles (UAVs) are becoming an integral part of both industry and society. In particular, the quadrotor is now invaluable across a plethora of fields and recent developments, such as the inclusion of aerial manipulators, only extends their versatility. As UAVs become more widespread, preventing loss-of-control (LOC) is an ever growing concern. Unfortunately, LOC is not clearly defined for quadrotors, or indeed, many other autonomous systems. Moreover, any existing definitions are often incomplete and restrictive. A novel metric, based on actuator capabilities, is introduced to detect LOC in quadrotors. The potential of this metric for LOC detection is demonstrated through both simulated and real quadrotor flight data. It is able to detect LOC induced by actuator faults without explicit knowledge of the occurrence and nature of the failure. The proposed metric is also sensitive enough to detect LOC in more nuanced cases, where the quadrotor remains undamaged but nevertheless losses control through an aggressive yawing manoeuvre. As the metric depends only on system and actuator models, it is sufficiently general to be applied to other systems.

==> notes.tex <==
Main thrust of paper:
- There is an elusive fragility which can affect quadrotors: these are the off-diagonal asymmetries which are typically ignored. 
- We show that with an aggressive controller, the quadrotor is able to reject the disturbances which manifest along these off-diagonals and accommodate them as they propagate to the main diagonal. Thus, we often do not see these issues arising. 
- However, ignoring them can lead to problems, even in hover. 
- Thus, we propose a semi-structured method for improving disturbance rejection. While only loop at a time, we already show improvements. Of course, this does not give guarantees for the full MIMO system, but this is something we plan to address in the future. 
- System bandwidth somewhere between 100-250 Hz (Model dynamics - sim frequency).


Scenario:
\begin{itemize}
% self.gains_inner_diag = np.array([18.3, 39.9, 3.8, 10], dtype = float)
% # self.gains_inner[:3, :3] = np.array([
% # [18.25412065,  2.93123791,  3.44539809],
% # [2.92265701, 39.87497986,  3.44383968],
% # [0.25002495,  0.24949734,  3.8331469]
% # ]).copy()
    \item Hover
    \item HD-Beetle-NGP009-Quadratic-Sym
    \item Input delay = 15 samples ($=0.06 s$) after 2 seconds
    \item $M_{x}$ disturbance (e.g. gust, moving arm, object drop etc.) of magnitude 0.01 Nm for duration of 1 second. Disturbance begins at 2 seconds. 
    \item This delay causes the nominal diagonal controller to lose control while the robustified controller is able to maintain control. 
    \item Of course, improvements can be made on the (robust) response. Nonetheless, the controller does not 'run away'.  
\end{itemize}

Next scenario: MaxVel/Circle/PosTrack with disturbance along manoeuvre

Realistic scenario: Change rotor constant of one of the motors (even though this changes dynamics a bit). 
















% Note: Even when rotated by 90 deg the quadrotor (HDBeeetle-NGP010-Quadratic-Sym) may still 'fall' in the same direction in the E-frame due to differences in the Fx and Fy models. So even if the moments induce the offset, since one model has more 'drag' it will cause an issue. 

% NOTE: What was I doing:
% LAPTOP -> Tuning PIDs for better response, added integrator stuff
% - TAKE LAPTOP PID CONTROLLER CLASS! 

% SSD - Investigating direction of 'fall' when rotation differently at the start
% -> It seems that the interplay between forces and moments causes rather upredictable motions. 
% It still doesn't really make sense to me since rotating it should not alter the behaviour of the system in isolation, the body dynamics remain the same. So why does it change? 
% The initial motions are induced by the moments 


==> reviewers.tex <==
\section{Reviewer comments}

\subsection{Reviewer 1 (ID 2):}
The paper introduces Loss of control (LOC) for UAV systems.
A novel metric, based on actuator capabilities, is
introduced to detect LOC in quadrotors. The potential of
this metric for LOC detection is demonstrated through both
simulated and real quadrotor flight data. 
The paper is well written, very interesting, mathematically
correct as far I can judge and interesting for the audience
of ICRA. I recommend acceptance of the paper.  


The main contribution of this paper is a novel indicator,
termed the feasibly controllable metric (FCM), that defines
LOC for quadrotors. By applying the proposed LOC detector
to both simulated and real flight data, the authors
demonstrate that the FCM is not only sensitive to LOC
detection under actuator faults, but is also capable of
detecting LOC when no faults are present (i.e. in the
undamaged case). Moreover, since the FCM derives from
system and actuator models, it is sufficiently general to
be compatible with other robotic or autonomous platforms
where such state measurements and suitable actuator models
are available.

Section II briefly describes the quadrotor equations of
motion
and aerodynamic models used in this study. The FCM metric
itself is derived in section III and applied to simulation
and
flight data in section IV.

The attached video is a good video. It clarifies the paper.
The quality is good. Once again, I recommend the acceptance
of the paper for ICRA conference. 




\subsection{Reviewer 2 (ID 6):}
This paper presents a novel metric to estimate the
loss-of-control (LOC) of a general dynamic system and tests
the proposed metric for a quadrotor case.
To calculate this metric, first, the error between the
expected and measured state derivative is computed.
Then the required control input change to bridge this gap
is computed and compared with the maximum control input
change the dynamic system can achieve.
In the case the input change cannot be achieved, the system
is deemed uncontrollable.
The corresponding metric is average over a moving window.
The proposed method is demonstrated in simulations and on
data corresponding to real quadrotor flights.

The paper is clearly presented, highlighting the novelty of
the proposed method, and clearly highlighting the
advantages and drawbacks of the proposed metric.
1- While the simulative results are quite clear, the
analysis related to the experimental data is less
conclusive.
2- It is expected that the $\dot{x}$ in the current system is
the angular acceleration. While I am expecting that the
authors are using the angular velocity to estimate the
angular acceleration, similar to the INDI control algorithm
they are using, this should have been mentioned.
3- Following the above point, is the filtration of the
measured states mentioned in section IV-C related to
filtering the already filtered angular acceleration, or is
it related to the filtration leading to the computation of
the angular acceleration? In the case of the latter,
doesn't this lead to a measurement that is substantially
lagging? How does this affect the FCM computation?
4- The paper is not well concluded.


\section{Action points}

\begin{enumerate}
    \item Clarify results of FCM metric with respect to experimental data
    \item Mention that, indeed, the rotational acceleration is derived from rotational velocity measurements (as is done with INDI)
    \item Clarify that, while there is a (2-4 sample) 'delay' introduced by estimating these rotational accelerations (and using the difference equation), we can compensate for this since we are using this purely for analysis (at this point in time). The goal is to label data such that we can train forecasters (on non-delayed signals!) to predict this labelled moment. Indeed, the FCM itself can be used in a control loop or as a feature for LOC forecasters, in which case this delay should be accommodated. Again, for LOC forecasters, a few milliseconds delay is negligible when compared to the window length of about 1 second. The only issues arise (as with INDI) when using it directly for control (i.e. to compensate errors), which is not the goal of the FCM. To purely detect LOC, this delay is not substantial and can be explicitly compensated for in some cases.
    \item Summarize conclusions more effectively. 
\end{enumerate}
